TryOnGAN: Body-Aware Try-On via Layered Interpolation

Given a pair of images-target person and garment on another person-we automatically generate the target person in the given garment. Previous methods mostly focused on texture transfer via paired data training, while overlooking body shape deformations, skin color, and seamless blending of garment with the person. This work focuses on those three components, while also not requiring paired data training. We designed a pose conditioned StyleGAN2 architecture with a clothing segmentation branch that is trained on images of people wearing garments. Once trained, we propose a new layered latent space interpolation method that allows us to preserve and synthesize skin color and target body shape while transferring the garment from a different person. We demonstrate results on high resolution 512x512 images, and extensively compare to state of the art in try-on on both latent space generated and real images.

==> 01_introduction.tex <==
\section{Introduction}

Virtual try-on—the ability to computationally visualize a garment of interest on a person of one’s choice—may become an essential part of an apparel shopping experience. A  useful  try-on, however, requires  high quality visualization, ideally indistinguishable from a photograph in a magazine with attention to body shape and type details. As a step towards this goal, we introduce a novel  image based try on algorithm, named \textit{TryOnGAN}, which seamlessly integrates person-specific components from one image with the garment shape and details from another image. Our experimental evaluation demonstrates state of the art photo-realistic results at the high resolution of $512\times512$ pixels.  
\begin{figure*}
    \centering \includegraphics[width=\textwidth]{figures/real-vs-generated-figure.png}
    \caption{Results from our method on real and generated images. We run the same optimization method on both types of images, with real image try-on requiring an additional projection step to the latent space.  On real images, our method generates high resolution try-on results  that accurately transform for body shape and synthesize skin consistent with identity. However, some garment details are lost in projection. On generated images, our method can accurately transfer complex garment textures and patterns in addition to correctly synthesizing identity details, e.g., hair, body shape, skin color. While texture details projection for real images is left for future work, our algorithm already as is outperforming state of the art.}
    \label{fig:real-vs-generated}
\end{figure*}

We are motivated by the photo-realism and high resolution results of StyleGAN \cite{StyleGAN,StyleGAN2} for faces, and use it as our starting point for fashion try-on. We design a modified StyleGAN2 network, conditioned on 2D human body pose with a clothing segmentation branch. This architecture is used to train a model on 100K \textbf{unpaired} fashion images. During test time, given a pair of images—a person image and a garment image— we propose a method that automatically searches for  optimal interpolation coefficients \textit{per layer}, such that, when applied on the two images result in try-on. Interpolation coefficients are applied on the latent representations of the two input images, and are used to generate a single output image where the person from the first input image is wearing the garment from the second image. Figures \ref{fig:teaser} and \ref{fig:real-vs-generated} demonstrate results on both real and generated images. Real image try-on requires an additional projection step ahead of the core algorithm. 

Per layer optimization  enables semantically meaningful and high quality results. Unlike previous general GAN editing methods \cite{Edo, NoiseInjection}, which require \textbf{manual} choice of noise injection structure or manual identification of clusters and fixed parameters for all layers, our method \textbf{automatically} computes the best interpolation coefficients per layer by optimizing a loss function designed to preserve the identity and body of the person while warping  only the garment. Results section shows comparison to \citet{Edo} and the importance of per layer optimization. 


Our method outperforms the state of the art \cite{ADGAN,CPVITON, ACGPN} with respect to three components: body shape, photorealism, and skin color preservation on real images, as well as generalizing to other datasets, while only using unpaired data.  While our method outperforms SOTA as it is, it can be further improved on real images to allow for complex texture patterns such as plaid, and specularities. We leave that for future work, for example, via improvement of projection to latent space which is an active research area in general GAN synthesis. We do demonstrate the full capabilities of our optimization method through try-on results on generated images. On generated images, our method can indeed further transfer high frequency details such as geometric patterns and complex textures, thus once latent space projection will be solved it will automatically apply to improve real images even further. 

Key contributions of this paper:
\begin{itemize}
    \item Photorealistic blend synthesis of person and garment (try-on) via StyleGAN interpolation algorithm using unpaired data.
    \item First method to allow for \textbf{body shape} deformation across the person and garment images.
    \item High quality synthesis of identity features and \textbf{body shape and skin color}. 
\end{itemize}

